Elucidating Interfacial Dynamics of Ti-Al Systems Using Molecular Dynamics Simulation and Markov State Modeling

Due to their remarkable mechanical and chemical properties, Ti-Al based materials are attracting considerable interest in numerous fields of engineering, such as automotive, aerospace, and defense. With their low density, high strength, and resistance to corrosion and oxidation, these intermetallic alloys and compound metal-metallic composites have found diverse applications. The present study delves into the interfacial dynamics of these Ti-Al systems, particularly focusing on the behavior of Ti and Al atoms in the presence of TiAl$_3$ grain boundaries under experimental heat treatment conditions. Using a combination of Molecular Dynamics and Markov State Model analyses, we scrutinize the kinetic processes involved in the formation of TiAl$_3$. The Molecular Dynamics simulation indicates that at the early stage of heat treatment, the predominating process is the diffusion of Al atoms towards the Ti surface through the TiAl$_3$ grain boundaries. The Markov State Modeling identifies three distinct dynamic states of Al atoms within the Ti/Al mixture that forms during the process, each exhibiting a unique spatial distribution. Using transition timescales as a qualitative measure of the rapidness of the dynamics, it is observed that the Al dynamics is significantly less rapid near the Ti surface compared to the Al surface. Put together, the results offer a comprehensive understanding of the interfacial dynamics and reveals a three-stage diffusion mechanism. The process initiates with the premelting of Al, proceeds with the prevalent diffusion of Al atoms towards the Ti surface, and eventually ceases as the Ti concentration within the mixture progressively increases. The insights gained from this study could contribute significantly to the control and optimization of manufacturing processes for these high-performing Ti-Al based materials.

==> contents/simulation_test.tex <==
To confirm and apply our findings to real-world problems, we simulate the heat treament of a Ti-Al alloy material after the direct energy deposition.

\subsection{Model setup and simulation details}
The simulation cell is defined as in \cref{fig:heat_treatment}. In this simulation cell, the top \SI{1}{\nano\meter}-thick layer of Ti and the bottom \SI{1}{\nano\meter}-thick layer of Al are fixed such that they are not allowed to move freely in the xy-plane while the movement along the z-axis is not constrained. A \SI{1}{\nano\meter}-wide margin of the TiAl\textsubscript{3} is fixed in all three direction, preventing the TiAl\textsubscript{3} layer (and thus the entire system) from floating freely in the space.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.6\textwidth]{figs/heat_treatment_sys}
    \caption{The simulation cell for the heat treatment process. Besides the dimensions shown in the figure, the thicknesses of the Al, TiAl\textsubscript{3} and Ti layers are \SI{10}{\nano\meter}, \SI{4}{\nano\meter} and \SI{4}{\nano\meter} respectively. The TiAl\textsubscript{3} layer consists of $4$ randomly oriented grains, forming grain boundaries. The lattice orientations of the Al and Ti layers are also random. (The supporting information includes all lattice oritentations.)}
    \label{fig:heat_treatment}
\end{figure}

The system is first equilibrated at \SI{300}{\kelvin} for \SI{1}{\nano\meter}. Then, it is heated up to \SI{895.15}{\kelvin} in \SI{300}{\pico\second}, corresponding to a heating rate of approximately \SI{2}{\kelvin/\pico\second}. Next, the system is kept at \SI{895.15}{\kelvin} for \SI{30}{\nano\second}. \SI{895.15}{\kelvin} falls in the temperature range identified in several experimental studies for Ti-Al intermetallic system annealing\cite{bizot2020reactivity, mirjalili2013kinetics, xu2006growth} and is a typical temperature used in this study\cite{mirjalili2013kinetics}. In the system of interest, at this temperature, the dominating dynamics is the diffusion of Al atoms from the pure Al side through the TiAl\textsubscript{3} grain boundaries to the Ti side. So, we analyze the evolution of the system by focusing on the diffusion of the Al atoms that originates from the pure Al layer (as opposed to the Al atoms originally in the TiAl\textsubscript{3}).
